Live Long and Prosper:Analyzing Long-Lived MOAS Prefixes in BGP

BGP exchanges reachability information in the form of prefixes, which are usually originated by a single Autonomous System (AS). If multiple ASes originate the same prefix, this is referred to as a Multiple Origin ASes (MOAS) prefix. One reason for MOAS prefixes are BGP prefix hijacks, which are mostly short-lived and have been studied extensively in the past years. In contrast to short-lived MOAS, long-lived MOAS have remained largely understudied. In this paper, we focus on long-lived MOAS prefixes and perform an in-depth study over six years. We identify around 24k long-lived MOAS prefixes in IPv4 and 1.4k in IPv6 being announced in January 2023. By analyzing the RPKI status we find that more than 40% of MOAS prefixes have all origins registered correctly, with only a minority of MOAS having invalid origins. Moreover, we find that the most prominent CIDR size of MOAS prefixes is /24 for IPv4 and /48 for IPv6, suggesting their use for fine-grained traffic steering. We attribute a considerable number of MOAS prefixes to mergers and acquisitions of companies. Additionally, more than 90% of MOAS prefixes are originated by two origin ASes, with the majority of detected origin AS relations being customer-provider. Finally, we identify that the majority of MOAS users are IT companies, and just 0.9% of IPv4 MOAS and 6.3% of IPv6 MOAS prefixes are used for anycast.

==> Makefile <==

# You want latexmk to *always* run, because make does not have all the info.
# Also, include non-file targets in .PHONY so they are run regardless of any
# file of the given name existing.
.PHONY: paper.pdf all clean

# The first rule in a Makefile is the one executed by default ("make"). It
# should always be the "all" rule, so that "make" and "make all" are identical.
all: paper.pdf

# CUSTOM BUILD RULES

# In case you didn't know, '$@' is a variable holding the name of the target,
# and '$<' is a variable holding the (first) dependency of a rule.
# "raw2tex" and "dat2tex" are just placeholders for whatever custom steps
# you might have.

#%.tex: %.raw
#        ./raw2tex $< > $@
#
#%.tex: %.dat
#        ./dat2tex $< > $@

# MAIN LATEXMK RULE

# -pdf tells latexmk to generate PDF directly (instead of DVI).
# -pdflatex="" tells latexmk to call a specific backend with specific options.
# -use-make tells latexmk to call make for generating missing files.

# -interaction=nonstopmode keeps the pdflatex backend from stopping at a
# missing file reference and interactively asking you for an alternative.

paper.pdf:
	latexmk -pdf -pdflatex="pdflatex -interaction=nonstopmode" -use-make $<

clean:
	latexmk -CA
	rm -vf *.bbl *.blg *.bcf *.run.xml

paper-gray.pdf: paper.pdf
	gs \
   	-sDEVICE=pdfwrite \
   	-sProcessColorModel=DeviceGray \
   	-sColorConversionStrategy=Gray \
   	-dOverrideICC \
   	-o paper-gray.pdf \
   	-f paper.pdf


manual:
	pdflatex paper.tex
	biber paper.bcf
	pdflatex paper.tex
	pdflatex paper.tex
	pdflatex paper.tex



==> include/acknowledgments.tex <==
\subsection*{Acknowledgements}

The authors would like to thank the anonymous reviewers and the shepherd Shep Herd for their thoughtful comments.


==> include/discussion.tex <==
%! TEX root = ../paper.tex
\section{Discussion}
\label{sec:discussion}
This discussion goes here




